Sinkhorn Natural Gradient for Generative Models

We consider the problem of minimizing a functional over a parametric family of probability measures, where the parameterization is characterized via a push-forward structure. An important application of this problem is in training generative adversarial networks. In this regard, we propose a novel Sinkhorn Natural Gradient (SiNG) algorithm which acts as a steepest descent method on the probability space endowed with the Sinkhorn divergence. We show that the Sinkhorn information matrix (SIM), a key component of SiNG, has an explicit expression and can be evaluated accurately in complexity that scales logarithmically with respect to the desired accuracy. This is in sharp contrast to existing natural gradient methods that can only be carried out approximately. Moreover, in practical applications when only Monte-Carlo type integration is available, we design an empirical estimator for SIM and provide the stability analysis. In our experiments, we quantitatively compare SiNG with state-of-the-art SGD-type solvers on generative tasks to demonstrate its efficiency and efficacy of our method.

==> Sinkhorn_information_matrix.tex <==
\section{Sinkhorn Information Matrix}
In this section, we derive the explicit expression of the \emph{Sinkhorn information matrix (SIM)} and show that it can be computed with logarithm times (in terms of the target accuracy) of simple function operations (e.g. $\log$ and $\exp$) and integration oracle queries.
The computability of SIM and hence SiNG shows the significant difference and advantage of SiNG over WNG and its variants, as they either are computationally tractable only under the $1$-dimensional parameterization or require unquantifiable approximation to the original update rule.
In the case when we can only compute the integration with respect to $\alpha_\theta$ in a Monte Carlo manner, 
an empirical estimator of SIM is proposed in the next section whose is consistency is then proved.

Note that $\SM(\cdot, \cdot)$ is the sum of the terms $\OTgamma(\cdot, \cdot)$. 
We hence focus on the term $\nabla^2_\theta \OTgamma(\alpha_{\theta}, \alpha_{\theta^t})_{\vert {\theta} = {\theta^t}}$ in $\HB(\theta^t)$. 
The other term $\nabla^2_\theta \OTgamma(\alpha_{\theta}, \alpha_{\theta})_{\vert {\theta} = {\theta^t}}$ can be handled in a similar manner and is deferred to the appendix.

Recall that the entropy regularized optimal transport distance $\OTgamma$ admits an equivalent dual concave-maximization form \eqref{eqn_OTepsilon_dual}.
Due to the concavity of $\HM_2$ w.r.t. $g$ in \eqref{eqn_OTepsilon_dual_two_variable}, for any fixed $f\in\CM(\XM)$, the corresponding optimal $g_f = \argmax_{g\in\CM(\XM)} \HM_2(f, g; \alpha, \beta)$ can be explicitly computed:
For a function $\bar f\in\CM(\XM)$ and a measure $\alpha\in\MM_1^+(\XM)$, define the Sinkhorn mapping as
\begin{equation} \label{eqn_sinkhorn_mapping}
	\AM[\bar f, \alpha] \defi -\gamma\log\int_\XM\exp\left\{-\frac{1}{\gamma}c(x, y) + \frac{1}{\gamma}\bar f(x)\right\}\dB\alpha(x).
\end{equation}
The first-order optimality of $g_f$ writes $g_f = \AM[f, \alpha]$.
Consequently, the dual potential variable problem \eqref{eqn_OTepsilon_dual} can be simplified to the following single potential variable problem
\begin{equation} \label{eqn_OTgamma_dual_single_variable}
	\OTgamma(\alpha_\theta, \beta) = \max_{f\in\CM(\XM)} \left\{\HM_1(f, \theta) \defi \langle f, \alpha_\theta\rangle + \langle \AM[f, \alpha_\theta], \beta\rangle  \right\},
\end{equation}
where in $\HM_1$ we emphasize the impact of $\theta$ to $\HM_1$ by writing it explicitly as a variable.
Besides, in $\HM_1$ the dependence on $\beta$ is dropped as $\beta$ is fixed.
Lastly, we denote the optimal solution to the R.H.S. of \eqref{eqn_OTgamma_dual_single_variable} by $f_\theta$ which is one of the Sinkhorn potentials to $\OTgamma(\alpha_\theta, \beta)$.

We will derive the explicit expression of $\nabla^2_\theta \OTgamma(\alpha_{\theta}, \alpha_{\theta^t})_{\vert {\theta} = {\theta^t}}$ based on the above dual representation.
%As $\HM_1$ involves operations on functions, we first formally define the Fr\'echet derivative. 
Recall the definition of the Fr\'echet derivative in Definition \ref{definition_frechet_derivative} and its chain rule $D(f\circ g)(x) = Df(g(x)) \circ Dg(x)$. We compute the first-order gradient by
\begin{equation}
	\nabla_\theta \OTgamma(\alpha_{\theta}, \beta) = \nabla_\theta \HM_1(f_\theta, \theta) = \underbrace{D_1 \HM_1(f_\theta, \theta)\circ Df_\theta}_{\GM_1(f_\theta, \theta)} + \underbrace{D_2 \HM_1(f_\theta, \theta)}_{\GM_2(f_\theta, \theta)},
\end{equation}
where $D_i\HM_1$ denote the Fr\'echet derivative of $\HM_1$ with respect to its $i^{th}$ variable.
Importantly, the optimality condition of \eqref{eqn_OTgamma_dual_single_variable} implies that $D_1 \HM_1(f_\theta, \theta)[g] = 0, \forall g\in\CM(\XM)$.\\
Further, in order to compute the second order gradient of $\OTgamma(\alpha_{\theta}, \beta)$ with respect to $\theta$, we first compute the gradient of $\GM_i, i=1,2$:
\begin{align}
	\nabla_\theta \GM_1(f_\theta, \theta) &\ = D_1 \HM_1(f_\theta, \theta)\circ D^2f_\theta + D^2_{11} \HM_1(f_\theta, \theta)\circ (Df_\theta, Df_\theta) + D^2_{12} \HM_2(f_\theta, \theta)\circ(Df_\theta, \IM_d), \label{eqn_frechet_derivative_i}\\
	\nabla_\theta \GM_2(f_\theta, \theta) &\ = D^2_{21}\HM_1(f_\theta, \theta)\circ(\IM, Df_\theta) + D^2_{22}\HM_1(f_\theta, \theta)\circ(\IM_d, \IM_d).
\end{align}
Using the fact that $D_1 \HM_1(f_\theta, \theta)[g] = 0, \forall g\in\CM(\XM)$, we can drop the first term in \eqref{eqn_frechet_derivative_i}.
Combining the above results, we have
\begin{equation}
	\begin{aligned}
	\nabla^2_\theta \OTgamma(\alpha_{\theta}, \beta) =\quad  &D^2_{11} \HM_1(f_\theta, \theta)\circ (Df_\theta, Df_\theta) + &D^2_{12} \HM_1(f_\theta, \theta)\circ(Df_\theta, \IM_d) \\
	+ &D^2_{21}\HM_1(f_\theta, \theta)\circ(\IM_d, Df_\theta) + &D^2_{22}\HM_1(f_\theta, \theta)\circ(\IM_d, \IM_d).
	\end{aligned}
\end{equation}
Since we have the explicit expression of $\HM_1$, the terms $D^2_{ij}\HM_1(f_\theta, \theta), i,j = 1,2$ can all be readily evaluated\footnote{We proved these expressions in the appendix.} once we have the integration oracle of $\alpha_\theta$ and $\beta$. 
Now we focus on $Df_\theta$, the Fr\'echet derivative of the implicit function $f_\theta$.

\noindent{\bf Computation and Convergence of the Sinkhorn Potential $f_\theta$.}
First, we recall existing results about the Sinkhorn potential $f_\theta$.
It is known that $f_\theta$ is a solution to the generalized DAD problem (eq. (7.4) in \cite{lemmens2012nonlinear}), which is the fixed point to the operator $\BM:\CM(\XM)\times\Theta\rightarrow\CM(\XM)$ defined as
\begin{equation} \label{eqn_main_fix_point}
	\BM[f, \theta] \defi \AM[\AM[f, \alpha_\theta], \beta].
\end{equation}
Further, from the Birkhoff-Hopf Theorem (Sections A.4 and A.7 in \cite{lemmens2012nonlinear}), we know that $\exp(\BM/\gamma)$ is a contraction operator under the Hilbert metric with a contraction factor $\lambda^2$ where $\lambda\defi\frac{1-\exp(M_c/\gamma)}{1+\exp(M_c/\gamma)}<1$ (see also Theorem B.5 in \cite{NIPS2019_9130}):
For strictly positive functions $f, f'\in\CM(\XM)$, define the Hilbert metric as $d_H(f, f') \defi \log \max_{x, y\in\XM} \frac{f(x) f'(y)}{f'(x) f(y)}$.
For any measure $\alpha\in\MM_1^+(\XM)$, we have
\begin{equation}\label{eqn_contraction_under_hilbert_metric}
	d_H(\exp(\AM[f, \alpha_\theta]/\gamma), \exp(\AM[f', \alpha_\theta]/\gamma))\leq \lambda d_H(\exp(f/\gamma), \exp(f'/\gamma)).
\end{equation}
Consequently, by applying the fixed point iteration
\begin{equation}
	f^{t+1} = \BM[f^t, \theta],
\end{equation}
also known as the Sinkhorn-Knopp algorithm,
%\footnote{For completeness, we provide a formal and detailed discuss of the above result in Appendix \ref{appendix_convergence_sinkhorn_knopp}.}
one can compute $f_\theta$ in logarithm time: $\|f^{t+1} - f_\theta\|_\infty=\OM(\lambda^t)$ (Theorem. 7.1.4 in \cite{lemmens2012nonlinear} and Theorem B.10 in \cite{NIPS2019_9130}).

\noindent{\bf Convergence of the Fr\'echet derivative $Df_\theta$.}
We now construct a sequence $\{g^t\}$ to approximate $Df_\theta$ such that for all $t\geq T(\epsilon)$ with some integer function $T(\epsilon)$, $\|g^t - Df_\theta\|_{op} \leq \epsilon$. We also show that $g^{T(\epsilon)}$ can be obtained in polynomial time.
For a given target accuracy $\epsilon>0$, denote $\bar \epsilon = \epsilon$. 
\begin{itemize}
	\item Use the Sinkhorn-Knopp algorithm to compute $\tilde f_\epsilon$, an approximation of $f_\theta$ such that $\|\tilde f_\epsilon-f_\theta\|_\infty\leq \bar \epsilon$. This computation can be done in $\OM(\log \frac{1}{\epsilon})$.
	\item Denote $\EM[f, \theta] = \BM[\cdots\BM[f, \theta]]$, the $l$ times composition of $\BM$ in its first variable. Pick $l = \lceil\log_{\lambda}\frac{1}{3}\rceil/2$, from the contraction of $\AM$ under the Hilbert metric \eqref{eqn_contraction_under_hilbert_metric}, we have
	\begin{align*}
		\|\EM[f, \theta] - \EM[f', \theta]\|_\infty &\ \leq \gamma d_H(\exp(\EM[f, \theta]/\gamma), \exp(\EM[f', \theta]/\gamma))\\
		&\ \leq \gamma\lambda^{2l} d_H(\exp(f/\gamma), \exp(f'/\gamma))\leq 2\lambda^{2l}\|f - f'\|_\infty \leq \frac{2}{3}\|f - f'\|_\infty,
	\end{align*}
	where we use $\|f - f'\|_\infty\leq d_H(\exp(f), \exp(f'))\leq 2\|f - f'\|_\infty$ in the first and third inequalities.
	Consequently, $\EM[\cdot, \theta]$ is a contraction operator under the $l_\infty$ norm and hence
	\begin{equation} \label{eqn_contraction_EM}
		||D^1\EM[f, \theta]\|_{op} \leq \frac{2}{3}.
	\end{equation}
	\item Given arbitrary initialization $g^0:\Theta\rightarrow T(\RBB^d, \CM(\XM))$\footnote{Recall that $T(\RBB^d, \CM(\XM))$ is the family of bounded linear operators from $\RBB^d$ to $\CM(\XM)$}, construct iteratively 
	\begin{equation}
		g^{t+1} = D_1\EM[\tilde f_\epsilon, \theta]\circ g^{t} + D_2\EM[\tilde f_\epsilon, \theta].
	\end{equation}
	We have that $\|g^{t+1} - Df_\theta\|_{op}\leq 3\epsilon + (\frac{2}{3})^t\|g^0 - Df_\theta\|_{op}$: Using the chain rule of the Fr\'echet derivative, we compute
	\begin{equation}
		Df_\theta = D_1\EM[f_\theta, \theta]\circ Df_\theta + D_2\EM[f_\theta, \theta].
	\end{equation}
	For any perturbation $h\in\RBB^d$ to $\theta$, we bound the difference of the directional derivatives by
	\begin{align*}
		&\ \|g^{t+1}[h] - Df_\theta[h]\|_\infty \\
		\leq&\ \|D_1\EM[f_\theta, \theta]\circ Df_\theta[h] - D_1\EM[\tilde f_\epsilon, \theta]\circ g^{t}[h]\|_\infty + \|D_2\EM[\tilde f_\epsilon, \theta][h] - D_2\EM[f_\theta, \theta][h]\|_\infty\\
		\leq&\ \frac{2}{3}\|Df_\theta[h] - g^{t}[h]\|_\infty + L\|\tilde f_\epsilon - f_\theta\|_\infty\|h\|_\infty \leq \frac{2}{3}\|Df_\theta - g^{t}\|_{op}\|h\|_\infty + \epsilon\|h\|_\infty,
	\end{align*}
	where in the second inequality we use the bound on $D_1\EM$ in \eqref{eqn_contraction_EM} and the \red{$L$-Lipschitz continuity of $D_2\EM$} with respect to its first argument.
	The above inequality is equivalent to 
	\begin{equation*}
		\|g^{t+1} - Df_\theta[h]\|_{op} - 3\epsilon \leq \frac{2}{3}\left(\|Df_\theta[h] - g^{t}\|_{op} - 3\epsilon \right) \Rightarrow \|g^{t+1} - Df_\theta[h]\|_{op}\leq 3\epsilon + (\frac{2}{3})^t\|g^0 - Df_\theta[h]\|_{op}.
	\end{equation*}
	Therefore, after $T(\epsilon) = \OM(\log\frac{1}{\epsilon})$ iterations, we find $g^{T(\epsilon)}$ such that $\|g^{T(\epsilon)} - Df_\theta\|_{op} \leq 4\epsilon$.
\end{itemize}



==> celebA_network.tex <==
----------------------------------------------------------------
        Layer (type)               Output Shape         Param #
================================================================
            Conv2d-1           [-1, 64, 32, 32]           4,800
         LeakyReLU-2           [-1, 64, 32, 32]               0
            Conv2d-3          [-1, 128, 16, 16]         204,800
       BatchNorm2d-4          [-1, 128, 16, 16]             256
         LeakyReLU-5          [-1, 128, 16, 16]               0
            Conv2d-6            [-1, 256, 8, 8]         819,200
       BatchNorm2d-7            [-1, 256, 8, 8]             512
         LeakyReLU-8            [-1, 256, 8, 8]               0
            Conv2d-9            [-1, 512, 4, 4]       3,276,800
      BatchNorm2d-10            [-1, 512, 4, 4]           1,024
        LeakyReLU-11            [-1, 512, 4, 4]               0
================================================================
Total params: 4,307,392
Trainable params: 4,307,392
Non-trainable params: 0
----------------------------------------------------------------
Input size (MB): 0.01
Forward/backward pass size (MB): 2.31
Params size (MB): 16.43
Estimated Total Size (MB): 18.76
----------------------------------------------------------------
----------------------------------------------------------------
        Layer (type)               Output Shape         Param #
================================================================
   ConvTranspose2d-1            [-1, 256, 4, 4]         262,144
       BatchNorm2d-2            [-1, 256, 4, 4]             512
              ReLU-3            [-1, 256, 4, 4]               0
   ConvTranspose2d-4            [-1, 128, 8, 8]         524,288
       BatchNorm2d-5            [-1, 128, 8, 8]             256
              ReLU-6            [-1, 128, 8, 8]               0
   ConvTranspose2d-7           [-1, 64, 16, 16]         131,072
       BatchNorm2d-8           [-1, 64, 16, 16]             128
              ReLU-9           [-1, 64, 16, 16]               0
  ConvTranspose2d-10            [-1, 3, 32, 32]           3,072
             Tanh-11            [-1, 3, 32, 32]               0
================================================================
Total params: 921,472
Trainable params: 921,472
Non-trainable params: 0


==> required.tex <==
\definecolor{myback}{RGB}{204,232,207}

\makeatletter
\newcommand{\AB}{\mathbf{A}}
\newcommand{\BB}{\mathbf{B}}
\newcommand{\CB}{\mathbf{C}}
\newcommand{\DB}{\mathbf{D}}
\newcommand{\EB}{\mathbf{E}}
\newcommand{\FB}{\mathbf{F}}
\newcommand{\GB}{\mathbf{G}}
\newcommand{\HB}{\mathbf{H}}
\newcommand{\IB}{\mathbf{I}}
\newcommand{\JB}{\mathbf{J}}
\newcommand{\KB}{\mathbf{K}}
\newcommand{\LB}{\mathbf{L}}
\newcommand{\MB}{\mathbf{M}}
\newcommand{\NB}{\mathbf{N}}
\newcommand{\OB}{\mathbf{O}}
\newcommand{\PB}{\mathbf{P}}
\newcommand{\QB}{\mathbf{Q}}
\newcommand{\RB}{\mathbf{R}}
\newcommand{\SB}{\mathbf{S}}
\newcommand{\TB}{\mathbf{T}}
\newcommand{\UB}{\mathbf{U}}
\newcommand{\VB}{\mathbf{V}}
\newcommand{\WB}{\mathbf{W}}
\newcommand{\XB}{\mathbf{X}}
\newcommand{\YB}{\mathbf{Y}}
\newcommand{\ZB}{\mathbf{Z}}
\newcommand{\zeroB}{\mathbf{0}}
\newcommand{\oneB}{\mathbf{1}}
\newcommand{\aB}{\mathbf{a}}
\newcommand{\bB}{\mathbf{b}}
\newcommand{\cB}{\mathbf{c}}
\newcommand{\dB}{\mathbf{d}}
\newcommand{\eB}{\mathbf{e}}
\newcommand{\fB}{\mathbf{f}}
\newcommand{\gB}{\mathbf{g}}
\newcommand{\hB}{\mathbf{h}}
\newcommand{\iB}{\mathbf{i}}
\newcommand{\jB}{\mathbf{j}}
\newcommand{\kB}{\mathbf{k}}
\newcommand{\lB}{\mathbf{l}}
\newcommand{\mB}{\mathbf{m}}
\newcommand{\nB}{\mathbf{n}}
\newcommand{\oB}{\mathbf{o}}
\newcommand{\pB}{\mathbf{p}}
\newcommand{\qB}{\mathbf{q}}
\newcommand{\rB}{\mathbf{r}}
\newcommand{\sB}{\mathbf{s}}
\newcommand{\tB}{\mathbf{t}}
\newcommand{\uB}{\mathbf{u}}
\newcommand{\vB}{\mathbf{v}}
\newcommand{\wB}{\mathbf{w}}
\newcommand{\xB}{\mathbf{x}}
\newcommand{\yB}{\mathbf{y}}
\newcommand{\zB}{\mathbf{z}}
\newcommand{\ZEROBB}{\mathbf{0}}
\newcommand{\ONEB}{\mathbf{1}}
\newcommand{\AM}{\mathcal{A}}
\newcommand{\AMB}{\mathbfcal{A}}
\newcommand{\BM}{\mathcal{B}}
\newcommand{\CM}{\mathcal{C}}
\newcommand{\DM}{\mathcal{D}}
\newcommand{\EM}{\mathcal{E}}
\newcommand{\FM}{\mathcal{F}}
\newcommand{\JM}{\mathcal{J}}
\newcommand{\PM}{\mathcal{P}}
\newcommand{\TM}{\mathcal{T}}
\newcommand{\UM}{\mathcal{U}}
\newcommand{\VM}{\mathcal{V}}
\newcommand{\XM}{\mathcal{X}}
\newcommand{\YM}{\mathcal{Y}}
\newcommand{\LM}{\mathcal{L}}
\newcommand{\NM}{\mathcal{N}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\OM}{\mathcal{O}}
\newcommand{\QM}{\mathcal{Q}}
\newcommand{\HM}{\mathcal{H}}
\newcommand{\IM}{\mathcal{I}}
\newcommand{\GM}{\mathcal{G}}
\newcommand{\SM}{\mathcal{S}}
\newcommand{\RM}{\mathcal{R}}
\newcommand{\ZM}{\mathcal{Z}}
\newcommand{\ZBB}{\mathbb{Z}}
\newcommand{\SBB}{\mathbb{S}}
\newcommand{\RBB}{\mathbb{R}}
\newcommand{\VBB}{\mathbb{V}}
\newcommand{\EBB}{\mathbb{E}}
\newcommand{\NBB}{\mathbb{N}}
\newcommand{\varepsilonM}{\mathcal{\varepsilon}}

\newcommand{\xT}{\tilde{\mathbf{x}}}
\newcommand{\yT}{\tilde{\mathbf{y}}}
\newcommand{\zT}{\tilde{\mathbf{z}}}
\newcommand{\dHat}{\hat{\mathbf{d}}}
\newcommand{\DHat}{\hat{\mathbf{D}}}
\newcommand{\xHat}{\hat{\mathbf{x}}}
\newcommand{\alphaB}{\mbox{\boldmath$\alpha$\unboldmath}}
\newcommand{\betaB}{\mbox{\boldmath$\beta$\unboldmath}}
\newcommand{\etaB}{\mbox{\boldmath$\eta$\unboldmath}}
\newcommand{\epsilonB}{\mbox{\boldmath$\epsilon$\unboldmath}}
\newcommand{\phiB}{\mbox{\boldmath$\phi$\unboldmath}}
\newcommand{\piB}{\mbox{\boldmath$\pi$\unboldmath}}
\newcommand{\PhiB}{\mbox{\boldmath$\Phi$\unboldmath}}
\newcommand{\PsiB}{\mbox{\boldmath$\Psi$\unboldmath}}
\newcommand{\thetaB}{\mbox{\boldmath$\theta$\unboldmath}}
\newcommand{\ThetaB}{\mbox{\boldmath$\Theta$\unboldmath}}
\newcommand{\muB}{\mbox{\boldmath$\mu$\unboldmath}}
\newcommand{\SigmaB}{\mbox{\boldmath$\Sigma$\unboldmath}}
\newcommand{\GammaB}{\mbox{\boldmath$\Gamma$\unboldmath}}
\newcommand{\LambdaB}{\mbox{\boldmath$\Lambda$\unboldmath}}
\newcommand{\lambdaB}{\mbox{\boldmath$\lambda$\unboldmath}}
\newcommand{\omegaB}{\mbox{\boldmath$\omega$\unboldmath}}
\newcommand{\DeltaB}{\mbox{\boldmath$\Delta$\unboldmath}}
\newcommand{\varepsilonB}{\mbox{\boldmath$\varepsilon$\unboldmath}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\find}{\mathop{\rm find}}
\newcommand{\rank}{\mathop{\rm rank}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\SPAN}{\mathbf{span}}
\newcommand{\sgn}{\mathrm{sgn}}
%\newcommand{\tr}{\mathrm{tr}}
\newcommand{\rk}{\mathrm{rank}}
\newcommand{\diag}{\mathsf{diag}}
\newcommand{\dg}{\mathsf{dg}}
\newcommand{\vect}{\mathsf{vec}}
\newcommand{\etal}{{\em et al.\/}\,}
\newcommand{\ie}{{\em i.e.\/}\,}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\prox}{\mathrm{prox}}
\newcommand{\defi}{{:=}}
\newcommand{\lk}{{l_k}}
\newcommand{\ik}{{i_k}}
\makeatother



\newcommand{\clr}[1]{{\color[rgb]{1,0,0} #1}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{lemma}{Lemma}[section]
%\newtheorem*{lemma*}{Lemma}
%\newtheorem*{theorem*}{Theorem}
%\newtheorem*{proposition*}{Proposition}
\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
